Knowledge Efficient Deep Learning for Natural Language Processing

Deep learning has become the workhorse for a wide range of natural language processing applications. But much of the success of deep learning relies on annotated examples. Annotation is time-consuming and expensive to produce at scale. Here we are interested in methods for reducing the required quantity of annotated data -- by making the learning methods more knowledge efficient so as to make them more applicable in low annotation (low resource) settings. There are various classical approaches to making the models more knowledge efficient such as multi-task learning, transfer learning, weakly supervised and unsupervised learning etc. This thesis focuses on adapting such classical methods to modern deep learning models and algorithms. This thesis describes four works aimed at making machine learning models more knowledge efficient. First, we propose a knowledge rich deep learning model (KRDL) as a unifying learning framework for incorporating prior knowledge into deep models. In particular, we apply KRDL built on Markov logic networks to denoise weak supervision. Second, we apply a KRDL model to assist the machine reading models to find the correct evidence sentences that can support their decision. Third, we investigate the knowledge transfer techniques in multilingual setting, where we proposed a method that can improve pre-trained multilingual BERT based on the bilingual dictionary. Fourth, we present an episodic memory network for language modelling, in which we encode the large external knowledge for the pre-trained GPT.

==> Chapters/memory.tex <==
\section{Enriching Pre-trained Models with Vector Quantized Memory Layer}

Recently, fine-tuning pre-trained deep language models, such as Generative Pre-Training (GPT)~\cite{radford2018improving} and Bidirectional Encoder Representations from
Transformers (BERT)~\cite{devlin2018bert}, has achieved remarkable success on various downstream natural language processing tasks. Since pre-trained deep models come out, it has inspired lots of follow up, most notably, we can categorize the follow ups into three different categories: 1) the model becomes deeper and deeper such as Nvidia's Megatron~\cite{shoeybi2019megatron}; 2) instead of pre-training a BERT like model which can only be used as an encoder, more and more work are trying to pre-train an unified seq2seq model which can be used for many downstream tasks, such as Google T5 and MASS~\cite{raffel2019exploring,song2019mass}; 3) there is increasing interest in pre-training multilingual model, such as multilingual BART~\cite{liu2020multilingual}.

We predict that pre-trained deep seq2seq multilingual models will become more and more popular and eventually will dominate the field. To train such a seq2seq model in unsupervised manner, denoise loss and its variations are widely used, i.e., given any input sequence, the model tries to recover itself from its corrupted version through encoder-decoder architecture. Naturally, this is a variational auto-encoder (VAE)~\cite{doersch2016tutorial} formulation. If the model is deep enough, then the decoder becomes too powerful, it will inevitably encounter the ``posterior collapse" problem~\cite{lucas2019understanding}, especially for low resource languages since deep model is easier to overfit under low-resource conditions. 

Additionally, for many problems, discrete representations are potentially a better fit. For example, language and speech are typically represented as a sequence of discrete symbols. Even pre-trained models have been widely used for a variety of downstream NLP tasks~\cite{liu2019fine,adhikari2019docbert}, however, to the best of our knowledge, they have not been studied extensively for tasks that really requires reasoning such as complex reasoning~\cite{chen2019deep} and predictive learning~\cite{oord2018representation}. To make the pre-trained models more suitable for the many of the tasks that really requires reasoning, we think discrete representations is a necessary component.

In this paper, we propose an approach that alleviate the problem of posterior collapse by combing the vector quantization and the pre-trained seq2seq model. Our model is easy to understand and simple to train. To the best of our knowledge, this is the first pre-trained seq2seq model that combining discrete representations. Additionally, it is the first discrete pre-trained model that get similar or slightly better performance as its continuous counterpart, while offering the flexibility of discrete representations.


\subsection{Related Work}

\subsubsection{Large Scale Pre-trained NLP Models}

Great success has been achieved by pre-training deep neural networks with language modeling and then fine-tuning the models on downstream tasks~\cite{radford2018improving,devlin2018bert,dong2019unified}. It significantly outperforms methods that use pre-trained language models as auxiliary features~\cite{peters2018deep}. Instead of using LSTM models~\cite{peters2018deep}, transformer~\cite{vaswani2017attention} has become a popular choice to capture long-range structures.

Since BERT~\cite{devlin2018bert} came out, lots of follow ups come out. We can categorize the follow ups into following categories: 1): the pre-trained models become deeper and deeper, from Megatron~\cite{shoeybi2019megatron} to Turing-NLG\footnote{https://www.microsoft.com/en-us/research/blog/turing-nlg-a-17-billion-parameter-language-model-by-microsoft/}. 2): instead of pre-training BERT model with fixed window size, several work try to train BERT variations to incorporate long term dependency such as XLNet~\cite{yang2019xlnet}. 3): pre-train smaller or compressed models while maintain the same or similar performance such as ALBERT~\cite{lan2019albert} 4): instead of training BERT which can be used as an encoder, pre-train an unified seq2seq model which can be used for many downstream tasks, like MASS, Google T5, BART and mBART~\cite{song2019mass,raffel2019exploring,lewis2019bart,liu2020multilingual}. For all those models, except training a monolingual model, we can also train a multilingual model.

Even BERT~\cite{devlin2018bert} is quite popular and has been successfully applied to many NLP applications, however, it's still difficult to be applied to tasks like machine translation and summarization that requires a decoder. Along with the increase of computing resource, there is a trend that pre-trained seq2seq model will dominate this field since it can be applied to many different tasks seamlessly. Moreover, multilingual pre-trained model will also be applied widely given the fact there are more than 200 languages in the world. In this section, we focus on the pre-trained multi-lingual seq2seq model.

\subsubsection{Vector Quantizated VAE and Memory Network}

VQ-VAE~\cite{van2017neural} is a generative model successfully combining the variational autoencoder framework with discrete latent representations. The motivation of VQ-VAE is to alleviate the ``posterior collapse" problem existed in many VAE models that have a powerful decoder. It use a posterior categorical distribution to model the latent variables in the variational auto-encoder. To do so, it applies vector quantization to latent variable, and it's simple to train. To some extend, we can think the vector quantization component is a special layer in the variational autoencoder.

Our approach is also somewhat inspired by memory network~\cite{weston2014memory}. 
Memory network has a memory module which can be learnt jointly with other components. It has shown success in different applications~\cite{kumar2016ask,na2017read,ma2018visual}.

The most related work to ours is product key memory network~\cite{guillaume2019large}. \citet{guillaume2019large} shows that it is possible to insert a large product key memory as a layer in a transformer architecture resulting a model where the same number of parameters and the same performance can be achieved with half the layers and with much faster training time than a standard transformer architecture. Here, we also follow this idea, but we don't use the product keys memory, instead, we use the vector quantization as that in~\citet{van2017neural} and our memory size is much larger. To accelerate the retrieval procedure, we use approximate nearest neighbor methods as that in Sparse Access Memory~\cite{rae2016scaling}.

% memory networks that employ some method of efficiently reading and writing to very large neural memories. This is done with.
% These large memories are used to providing additional model capacity where the memory contents are trained over a large data set using gradient descent training, just as one would train the parameters of a very large network.


\subsection{Model}

In this section, we will introduce our model. First, we will introduce the memory network, which is a high level overview of the product keys memory network~\cite{guillaume2019large}. Then we will introduce the vector quantization technique we used in this paper. Finally, we will introduce our final model, which is a combination of those two. 

\smallpar{Memory Network}

The overall structure of product keys memory network is illustrated in Figure \ref{fig:memory_network}. A typical transformer block is composed by a self-attention layer followed by a two layer feed forward neural network (FFN). \citet{guillaume2019large} replaces the FFN layer with a product key memory layer, which is analogous to a sparse FFN layer with a very large hidden state representation. 

\begin{figure}[!htbp]
   \begin{center}
   \includegraphics[width=0.49\textwidth]{Figures/model.png}
   \end{center}
 \caption{An overview of the product keys memory network.}
 \label{fig:memory_network}
\end{figure}

\citet{guillaume2019large} uses product keys memory in memory layer. The memory layer contains three components: a query network, a key selection module, and a value lookup table where each value corresponds to one key. Given input representation, it first computes a query representation that is compared to all keys. For each key, it computes a score and selects the $k$ product keys with the highest scores. To produce an output representation $m(x)$, it uses a weighted sum over the values associated with the selected keys. 

Specifically, in implementation, the query network contains MLP followed by a batch normalization layer. Mathematically, it's a function $q: x \rightarrow q(x) \in R^{d_{q}}$ that maps the $d$ dimensional input $x$ to a latent space with dimensionality $d_{q}$.  

For the key selection and value lookup table, let $q(x)$ be a query and $\Gamma_{k}$ denote the top-$k$ operator. Given a set of keys $\mathcal{K}=\{ k_{1},\ldots, k_{|\mathcal{K}|}\} $ composed of $|\mathcal{K}|$ $d_{q}$-dimensional vectors, and an input representation $x$, they select the top $k$ keys maximizing the inner product with the query $q(x)$:
\begin{eqnarray*}
\mathcal{I}&=&\Gamma_{k}(q(x)^{T}k_{i}), 1 \leq i \leq |\mathcal{K}|\\
w&=&\text{Softmax}_{{i \in \mathcal{I}}}\quad q(x)^{T}k_{i},\\
m(x)&=&\sum_{i \in {\mathcal{I}}} w_{i}v_{i}
\end{eqnarray*}

To efficiently calculate the top-$k$ keys, they use the product key structure which can reduce the search complexity from $O(|\mathcal{K}| \times d_{q})$ to $O(\sqrt{|\mathcal{K}|} \times d_{q})$, and this is one of the key contribution in~\citet{guillaume2019large}.

For multiple layer transformer, they will replace the FFN layer with the memory layer in several layers. For multiple heads, each head independently computes a query vector used to select $k$ keys from the memory, the final memory sums the output $m_{i}(x)$ of each head $i$: $m(x) = \sum_{i=1}^{H}m_{i}(x)$ where $H$ is the number of heads.

All the parameters of the memory layer are trainable, and the sparse selection and parameter updating make both training and inference very efficient. More details are given in~\citet{guillaume2019large}.

\smallpar{Vector Quantization VAE}
 
 The core contribution of VQ-VAE~\cite{van2017neural} is adding a vector quantization layer between the encoder and decoder. Given the query vector $q(x)$ (encoder's output), and $e \in R^{K \times d_{q}}$ is a latent embedding space where $K$ is the size of the discrete latent space, and dimensionality of each latent embedding vector $e_{i}$ equals to the query vector's dimensionality $d_{q}$. Given $q(x)$, it's passed through the vector quantization layer by mapping the query $q(x)$ to the nearest element of embedding:
 \begin{equation}
 m(x) = e_{k}, \text{where } k = \arg\min_{j} \| q(x) - e_{j} \|_{2}    
 \label{eqn:vq}
 \end{equation}
 
 There is no exact gradient for Equation \ref{eqn:vq} due to $\arg\min$ operator. To train the model, the VQ-VAE approximates the gradient similar to the straight-through estimator and copy gradients from decoder input $m(x)$ to encoder output $q(x)$, and the final loss is:
 \begin{eqnarray*}
 \mathcal{L} = \log p(x|m(x)) + \| \text{sg}(q(x)) - e \|_{2}^{2} \\
 + \beta \| q(x) - \text{sg}(e) \|_{2}^{2}    
 \label{eqn:loss}
 \end{eqnarray*}
 where $\text{sg}$ means stop gradient. Through straight-through estimator, the gradient from the task loss can also be propagated to the encoder.
 
 The product keys memory network is only used as encoder~\cite{guillaume2019large}, and in vector quantization VAE~\cite{van2017neural}, vector quantization is only applied to the encoder's output. In this paper, we aim at alleviating the posterior collapse issue for large scale pre-trained model, thus we can apply the vector quantization to multiple layers in both encoder and decoder, further, we can also discretize the encoder's output, as illustrated in Figure \ref{fig:overall}.
 
\begin{figure*}[!htbp]
   \begin{center}
   \includegraphics[width=0.98\textwidth]{Figures/overview.png}
   \end{center}
 \caption{An overview of our final model.}
 \label{fig:overall}
\end{figure*}

In our model, we use multiple vector quantization layers, thus we need to use straight-through gradient estimator for each vector quantizated layer, similarly, we also need to calculate $\| \text{sg}(q(x)) - e \|_{2}^{2} + \beta \| q(x) - \text{sg}(e) \|_{2}^{2}$ multiple times.

\subsection{Experiments}


  We primarily focus on vector quantized seq2seq learning. First, we pre-train vector quantized seq2seq models from scratch to demonstrate the idea, then we apply the vector quantization to large scale pre-trained models. For seq2seq models, we try several different pre-trained models such as MASS~\cite{song2019mass}, Google T5~\cite{raffel2019exploring} and mBART~\cite{liu2020multilingual}. Those models have different training criterion, by applying the vector quantization to all of them, we can check whether our vector quantization is orthogonal to specific training criterion. We will introduce those models in section \ref{sec:pre-trained_model}.
  
  Since we don't have too much GPU resources, we first train small seq2seq models to demonstrate the vector quantization idea, then we take off-the-shell pre-trained models, augment it with additional vector quantization layers and then fine tune it on downstream tasks. When fine tune the released pre-trained models on downstream tasks, we pay special attention to their multilingual version since the deep seq2seq models are easier to overfit to low resource languages. We will introduce downstream tasks we considered in section \ref{sec:downstream_task}.  
  
  
\subsubsection{Pre-trained Models}
\label{sec:pre-trained_model}
 
  Before going to the details, we first briefly introduce three pre-trained models here: MASS~\cite{song2019mass}, Google T5~\cite{raffel2019exploring} and mBART~\cite{liu2020multilingual}. 
  
  \textbf{MASS}: MASS~\cite{song2019mass} adopts the encoder-decoder framework to reconstruct a sentence fragment given the remaining part of the sentence. Its encoder takes a sentence with randomly masked fragment (several consecutive tokens) as input, and its decoder tries to predict this masked fragment. In this way, MASS can jointly train the encoder and decoder to do representation extraction and language modeling. 
  
  \textbf{Google T5}: Google T5~\cite{raffel2019exploring} adopts the encoder-decoder framework and systematically compares pre-training objectives, architectures, unlabeled datasets, transfer approaches, and other factors on dozens of language understanding tasks. Due to computing resource limit, we will only use the following three released models: T5-small, T5-base and T5-large. 
  
  \textbf{mBART}: mBART~\cite{liu2020multilingual} is a multilingual version of BART~\cite{lewis2019bart}. BART pre-trains a seq2seq model combining bidirectional and auto-regressive transformer. It first corrupts text with an arbitrary noising function and then learn a seq2seq model to reconstruct the original text. The key insight is the noising function's flexibility, and eventually arbitrary transformations can be applied to the original text. The corruption operations they considered are: token masking, token deletion, text infilling, sentence permutation and document rotation.
  
  
\subsubsection{Downstream Tasks}
\label{sec:downstream_task}
   
  When fine tune, we consider NLP applications such as sequence classification, token classification, sequence generation and machine translation. For all those tasks, we consider the corresponding multilingual datasets.
  
  \noindent\textbf{Sequence classification}: we consider cross-lingual natural language inference (NLI), and we choose XNLI corpus~\cite{conneau2018xnli}. XNLI consists of 7,500 human-annotated dev/test examples spread in a variety of language families. XNLI has three experiment settings: \textit{translate train}, \textit{translate test}, and \textit{zero shot}. 
  
  
  \noindent\textbf{Token classification}: we consider the machine translation quality estimation and cross lingual extractive question answering. For machine translation quality estimation, we use Task $2$ -- word-level quality estimation in WMT18~\cite{wmt2018}. Given a source sentence and its translation (target), it aims to estimate the translation quality (\emph{``BAD"} or \emph{``OK"}) at each position: each token in the source and target sentence, each gap in the target sentence. For cross lingual extractive question answering, we choose MLQA dataset~\cite{lewis2019mlqa}, which is a multilingual version of SQuAD~\cite{rajpurkar2016squad}.
  
  
  \noindent\textbf{Sequence generation}: we consider cross lingual summarization. We use large-scale cross lingual summerization (CLS) dataset from~\citet{zhu2019ncls}. It contains a 370K English-to-Chinese (En2Zh) and CLS corpus and a 1.69M Chinese to English (Zh2En) CLS corpus. 
  
  \noindent\textbf{Machine translation}: we consider supervised machine translation (MT) and low resource machine translation. For low resource machine translation, we pay special attention to unsupervised MT.
  

\subsubsection{Experimental Results}

\textbf{Pre-training Experiments}
 
 We pre-train seq2seq learning models with vector quantization layer. Due to GPU resource limit, we only train small seq2seq model with 3 layers and 6 heads. The embedding dimension is 384, the layer 1 is memory layer with memory size 50000, and we use batch normalization after the query network. We consider English and French, for each language, we randomly choose 10M sentences from the WMT monolingual News Crawl datasets from years 2007 through 2013 and concatenate them. We use Moses scripts~\cite{koehn2007moses} for tokenization. We use fastBPE to learn the joint BPE codes with codes size is 60,000. We evaluate the perplexity on en-fr WMT newstest 2014. The result is given in Table  \ref{tab:pre-training_result}.

\begin{table}[h!t]
\footnotesize
\centering
  \begin{tabular}{lcc}
    \toprule
    \textbf{Model} & \textbf{Dev} & \textbf{Test} \\ 
    \midrule
    en &  &  \\
    \midrule
    Transformer &  269.99 &   259.10 \\
    Transformer+Memory Layer & 268.52 & 259.68 \\
    Transformer+VQ Memory Layer & \textbf{262.29} & \textbf{252.75} \\
    \midrule
    fr &  &  \\
    \midrule
    Transformer &  \textbf{215.03} &  \textbf{199.60} \\
    Transformer+Memory Layer &  217.05 & 202.53 \\
    Transformer+VQ Memory Layer & 215.10 & 199.69 \\
    \bottomrule
  \end{tabular}
\caption{Perplexity with different models using MASS criterion.}
\label{tab:pre-training_result}
\end{table}

\textbf{Fine Tune Experiments}
\vspace{1em}


\smallpar{Sequence Classification}

\smallpar{Token Classification}

\smallpar{Sequence Generation}

\smallpar{Machine Translation}


==> Chapters/parser.tex <==
\section{Parser}

==> discussion.tex <==
\section{Discussion}


==> name.tex <==
\renewcommand\makesign{
  \btypeout{Title Page}
  \hypersetup{pdftitle={\@title}}
  \hypersetup{pdfsubject=\subjectname}
  \hypersetup{pdfauthor=\authornames}
  \hypersetup{pdfkeywords=\keywordnames}
  \thispagestyle{empty}
  \begin{titlepage}
    \let\footnotesize\small
    \let\footnoterule\relax
    \let \footnote \thanks
    \setcounter{footnote}{0}
    \null\vfil
    \vskip 60\p@
    \begin{center}
      \setlength{\parskip}{0pt}
      %{\large\textbf{\UNIVNAME}\par}
      %\vfill
      {\huge \bf Knowledge Efficient Deep Learning for Natural Language Processing \par}
      \vfill
      {\LARGE by \par}
      \smallskip
      {\LARGE \authornames \par}
      \vfill
      {\LARGE A thesis submitted in partial fulfillment for the degree of \par}
      \vfill
      {\LARGE Doctor of Philosophy in Computer Science \par}
      \bigskip
      {\LARGE at the \par}
      {\LARGE \facname \par}
      {\LARGE \deptname \par}
      {\LARGE Chicago, Illinois \par}
      \bigskip
      \bigskip
      \bigskip
      {\LARGE Thesis Committee: \par}
      {\LARGE
        \begin{tabular}[t]{lll}
	Dr. David McAllester & Signed: \rule[0em]{6em}{0.5pt} & Date: \rule[0em]{6em}{0.5pt} \\
	Dr. Kevin Gimpel & Signed: \rule[0em]{6em}{0.5pt} & Date: \rule[0em]{6em}{0.5pt} \\
	Dr. Hoifung Poon & Signed: \rule[0em]{6em}{0.5pt} & Date: \rule[0em]{6em}{0.5pt}
        \end{tabular}
      \par}
      
      %{\LARGE Dr. David McAllester (Thesis Advisor) Signed: \rule[1em]{15em}{0.5pt} Date: \rule[1em]{15em}{0.5pt}  \par}
      %{\LARGE Dr. Kevin Gimpel, TTIC \par}
      %{\LARGE Dr. Hoifung Poon, Microsoft Research \par}
      \bigskip
      {\LARGE \@date \par}
      \bigskip
    \end{center}
    \par
    \@thanks
    \vfil\null
  \end{titlepage}
  \setcounter{footnote}{0}%
  \global\let\thanks\relax
  \global\let\maketitle\relax
  \global\let\@thanks\@empty
  \global\let\@author\@empty
  \global\let\@date\@empty
  \global\let\@title\@empty
  \global\let\title\relax
  \global\let\author\relax
  \global\let\date\relax
  \global\let\and\relax
  \cleardoublepage
}



